Classification and Analysis of Communication Protection Policy Anomalies

This paper presents a classification of the anomalies that can appear when designing or implementing communication protection policies. Together with the already known intra- and inter-policy anomaly types, we introduce a novel category, the inter-technology anomalies, related to security controls implementing different technologies, both within the same network node and among different network nodes. Through an empirical assessment, we prove the practical significance of detecting this new anomaly class. Furthermore, this paper introduces a formal model, based on first-order logic rules that analyses the network topology and the security controls at each node to identify the detected anomalies and suggest the strategies to resolve them. This formal model has manageable computational complexity and its implementation has shown excellent performance and good scalability.

==> entities100.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
100;100;21;440;833;3036.67;4019.67
100;150;21;984;852.67;6467.67;7320.33
100;200;21;1744;837;11358.33;12195.33
100;250;21;2720;967;17906.67;18873.67
100;300;21;3912;988;26021.33;27009.33
100;350;21;5320;1056.33;35546.33;36602.67
100;400;21;6944;1134.33;46425;47559.33
100;450;21;8784;1228.33;60120.33;61348.67
100;500;21;10840;1305;74050.33;75355.33


==> entities250.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
250;100;36;440;1804;3157.33;4961.33
250;150;36;984;1841;7140.33;8981.33
250;200;36;1744;1934.33;12689.67;14624
250;250;36;2720;1988.67;20004.67;21993.33
250;300;36;3912;2070.33;29207.67;31278
250;350;36;5320;2147.33;40407;42554.33
250;400;36;6944;2236;52373.33;54609.33
250;450;36;8784;2278.67;67223;69501.67
250;500;36;10840;2352.33;82201.67;84554


==> entities500.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
490;100;60;440;4343.67;3799.33;8143
490;150;60;984;4450;8534;12984
490;200;60;1744;4493;15191.33;19684.33
490;250;60;2720;4599;23725.33;28324.33
490;300;60;3912;4669.33;34705.33;39374.67
490;350;60;5320;4706.67;47523;52229.67
490;400;60;6944;4769;62236;67005
490;450;60;8784;4857.67;80080;84937.67
490;500;60;10840;4894;98952;103846


==> pis100.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
50;100;16;440;1087;3028.33;4225.33
100;100;21;440;1195.67;3240.33;4426
150;100;26;440;1367.67;3187.67;4555.33
200;100;31;440;1544.67;3269;4813.67
250;100;36;440;2039.33;3250;5209.33
300;100;41;440;2444.33;3434.33;6078.67
350;100;46;440;2922.33;3587.67;6510
400;100;51;440;3398.33;3623;6941.33
450;100;56;440;3957.67;3770;7761.67
500;100;61;440;4607.33;3882.67;8440


==> pis250.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
50;250;16;2720;665.33;17992;18957.33
100;250;21;2720;915;18596.67;19511.67
150;250;26;2720;1242.67;18921.33;20154
200;250;31;2720;1633;19243.33;20876.33
250;250;36;2720;2038.33;20697.67;22536
300;250;41;2720;2516.67;20925.33;23442
350;250;46;2720;3006.33;22130;25136.33
400;250;51;2720;3551.33;22344;26095.33
450;250;56;2720;4170.33;23788.67;27659
500;250;61;2720;4758.33;24064.67;28823


==> pis500.tex <==
Ent; PI; Node; C; tp; tc; tp+tc
50;500;16;10840;1024.67;72900.67;73925.33
100;500;21;10840;1289.67;75472.33;76762
150;500;26;10840;1638;78149.67;79787.67
200;500;31;10840;1960;82102.33;84162.33
250;500;36;10840;2409;83774.33;86383.33
300;500;41;10840;2865.33;88153.67;90419
350;500;46;10840;3323.67;90099.67;93423.33
400;500;51;10840;3895;93108;97003
450;500;56;10840;4440.33;96438.67;100879
500;500;61;10840;5097;100933.33;107090.33

